RESTA: Time-Scaling Augmentation for Data-Efficient Robot Imitation Learning

Robot manipulation policies trained through imitation learning commonly rely on costly demonstrations recorded in one task direction and at one temporal resolution. We propose Reversal and Stride-based Trajectory Augmentation (RESTA), which exploits time-scaling data augmentation to improve data efficiency through trajectory reversal and temporal resampling. Trajectory-reversal augmentation reverses and relabels demonstrations between paired tasks with opposite objectives, reusing recorded rollouts without additional environment interaction. Because contact-rich manipulation is not exactly reversible, we treat reversal as an approximate paired-task prior rather than a physical symmetry. Temporal-stride augmentation varies observation and action sampling strides and conditions the policy on the resulting offsets, enabling fixed or randomized temporal schedules. Experiments across 16 paired bimanual manipulation tasks show that trajectory reversal is particularly effective in the low-data regime and that temporal-stride augmentation improves success under randomized temporal schedules. With 25 and 50 independently collected demonstrations per task, RESTA achieves 78.4% and 85.2% average success, respectively, matching or exceeding baselines trained with twice as many demonstrations (77.3% and 85.4%). These results show that RESTA can improve data efficiency in robot imitation learning.

==> result_tables.tex <==
% Experimental-results tables (3,000-epoch checkpoints only).
% Required package: \usepackage{booktabs}
%
% All entries are task success rates over 100 evaluation episodes. The paired
% 16-task suite excludes the two container-plate tasks from the older 18-task
% ablation. B_n denotes a baseline trained with n native trajectories; other
% short method names are defined in the corresponding captions.

% 1. Effect of time-reversal augmentation (n = 25 and n = 50).
\begin{table*}[t]
    \centering
    \caption{Effect of time-reversal augmentation at 3,000 training epochs.
    $B_n$ is the baseline trained with $n$ native trajectories, and
    $\mathrm{TR}_n$ (TR, time reversal) is trained with $n$ native and $n$ time-reversed
    trajectories. Thus, $B_{2n}$ controls for the total number of
    trajectories in $\mathrm{TR}_n$. Values
    are success rates (\%).}
    \label{tab:time-reversal-effect}
    \setlength{\tabcolsep}{7pt}
    \begin{tabular}{lccccc}
        \toprule
        Task & $B_{25}$ & $\mathrm{TR}_{25}$ & $B_{50}$ & $\mathrm{TR}_{50}$ & $B_{100}$ \\
        \midrule
        Place Fan            & 23 & 34  & 34  & 58  & 65  \\
        Remove Fan           & 87 & 82  & 92  & 85  & 99  \\
        Place Object Stand   & 43 & 61  & 61  & 72  & 80  \\
        Remove Object Stand  & 64 & 67  & 82  & 80  & 87  \\
        Place Empty Cup      & 47 & 83  & 77  & 74  & 93  \\
        Remove Empty Cup     & 91 & 94  & 90  & 98  & 100 \\
        Hang Mug             & 19 & 27  & 24  & 28  & 31  \\
        Unhang Mug           & 79 & 77  & 96  & 76  & 94  \\
        Rotate QR Code       & 55 & 55  & 69  & 78  & 75  \\
        Rotate QR Code Back  & 99 & 98  & 100 & 100 & 98  \\
        Handover Block       & 86 & 92  & 89  & 94  & 97  \\
        Handover Block Back  & 99 & 100 & 97  & 97  & 99  \\
        Open Laptop          & 70 & 81  & 85  & 81  & 86  \\
        Close Laptop         & 73 & 61  & 88  & 73  & 88  \\
        Open Microwave       & 72 & 83  & 80  & 73  & 92  \\
        Close Microwave      & 73 & 77  & 73  & 69  & 83  \\
        \midrule
        Macro average        & 67.5 & 73.3 & 77.3 & 77.2 & 85.4 \\
        \bottomrule
    \end{tabular}
\end{table*}

% 2. Effect of TSA and observation-offset conditioning (n = 50).
\begin{table*}[t]
    \centering
    \caption{Effect of temporal-stride augmentation and observation-offset
    conditioning on all 16 paired tasks at 3,000 training epochs.
    $B_{50}$ is the baseline, $\mathrm{TSA}_{50}$ (TSA, temporal stride
    augmentation) adds temporal-stride
    augmentation, and $\mathrm{TSAO}_{50}$ adds temporal-stride augmentation
    with observation offset. $\mathrm{TSA}_{50}$ and $\mathrm{TSAO}_{50}$ use
    randomized stride schedules. Values are success rates (\%).}
    \label{tab:tsa-oo-effect}
    \begin{tabular}{lccc}
        \toprule
        Task & $B_{50}$ & $\mathrm{TSA}_{50}$ & $\mathrm{TSAO}_{50}$ \\
        \midrule
        Place Fan           & 34 & 30 & 38 \\
        Remove Fan          & 92 & 100 & 100 \\
        Place Object Stand  & 61 & 67 & 67 \\
        Remove Object Stand & 82 & 81 & 85 \\
        Place Empty Cup     & 77 & 80 & 85 \\
        Remove Empty Cup    & 90 & 97 & 99 \\
        Hang Mug            & 24 & 22 & 28 \\
        Unhang Mug          & 96 & 95 & 96 \\
        Rotate QR Code      & 69 & 76 & 79 \\
        Rotate QR Code Back & 100 & 99 & 99 \\
        Handover Block      & 89 & 93 & 97 \\
        Handover Block Back & 97 & 99 & 98 \\
        Open Laptop         & 85 & 90 & 97 \\
        Close Laptop        & 88 & 88 & 93 \\
        Open Microwave      & 80 & 95 & 95 \\
        Close Microwave     & 73 & 81 & 75 \\
        \midrule
        Macro average       & 77.3 & 80.8 & 83.2 \\
        \bottomrule
    \end{tabular}
\end{table*}

% 3. Observation-offset ablation with time-reversed trajectories.
\begin{table*}[t]
    \centering
    \caption{Observation-offset ablation at 3,000 training epochs. $B_n$ is
    the baseline trained with $n$ native trajectories, and
    $\methodname{}_n$ (combining time reversal with temporal
    stride augmentation and observation offset) combines $n$ native and $n$ reversed
    trajectories with temporal-stride augmentation and observation offset
    using a
    randomized stride schedule. $B_{2n}$ controls for the total number of
    trajectories in $\methodname{}_n$. Values are success rates (\%).}
    \label{tab:fr-tsa-oo-ablation}
    \setlength{\tabcolsep}{7pt}
    \begin{tabular}{lccccc}
        \toprule
        Task & $B_{25}$ & $\methodname{}_{25}$ & $B_{50}$ & $\methodname{}_{50}$ & $B_{100}$ \\
        \midrule
        Place Fan            & 23 & 43  & 34  & 55  & 65  \\
        Remove Fan           & 87 & 96  & 92  & 99  & 99  \\
        Place Object Stand   & 43 & 58  & 61  & 79  & 80  \\
        Remove Object Stand  & 64 & 75  & 82  & 76  & 87  \\
        Place Empty Cup      & 47 & 77  & 77  & 91  & 93  \\
        Remove Empty Cup     & 91 & 97  & 90  & 100 & 100 \\
        Hang Mug             & 19 & 25  & 24  & 36  & 31  \\
        Unhang Mug           & 79 & 72  & 96  & 85  & 94  \\
        Rotate QR Code       & 55 & 80  & 69  & 88  & 75  \\
        Rotate QR Code Back  & 99 & 100 & 100 & 99  & 98  \\
        Handover Block       & 86 & 92  & 89  & 96  & 97  \\
        Handover Block Back  & 99 & 100 & 97  & 99  & 99  \\
        Open Laptop          & 70 & 93  & 85  & 97  & 86  \\
        Close Laptop         & 73 & 69  & 88  & 92  & 88  \\
        Open Microwave       & 72 & 96  & 80  & 98  & 92  \\
        Close Microwave      & 73 & 82  & 73  & 74  & 83  \\
        \midrule
        Macro average        & 67.5 & 78.4 & 77.3 & 85.2 & 85.4 \\
        \bottomrule
    \end{tabular}
\end{table*}

% 4. Main comparison (n = 25 and n = 50).
\begin{table*}[t]
    \centering
    \caption{Main results on all 16 paired tasks at 3,000 training epochs.
    $B_n$ is the $n$-trajectory baseline, $\mathrm{TR}_n$ (TR, time reversal) uses $n$ native
    and $n$ reversed trajectories, and $\methodname{}_n$ additionally
    applies temporal-stride augmentation with observation offset using a
    randomized stride schedule. The $\mathrm{TSAO}_{25}$ and
    $\mathrm{TSAO}_{50}$ columns report the randomized-offset (rand)
    evaluations.
    Values are success rates (\%).}
    \label{tab:main-results}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{lccccccccc}
        \toprule
        Task & $B_{25}$ & $\mathrm{TR}_{25}$ & $\mathrm{TSAO}_{25}$ & $\methodname{}_{25}$ & $B_{50}$
             & $\mathrm{TR}_{50}$ & $\mathrm{TSAO}_{50}$ & $\methodname{}_{50}$ & $B_{100}$ \\
        \midrule
        Place Fan            & 23 & 34  & 30 & 43  & 34  & 58  & 38  & 55  & 65  \\
        Remove Fan           & 87 & 82  & 100 & 96  & 92  & 85  & 100 & 99  & 99  \\
        Place Object Stand   & 43 & 61  & 50 & 58  & 61  & 72  & 67  & 79  & 80  \\
        Remove Object Stand  & 64 & 67  & 68 & 75  & 82  & 80  & 85  & 76  & 87  \\
        Place Empty Cup      & 47 & 83  & 71 & 77  & 77  & 74  & 85  & 91  & 93  \\
        Remove Empty Cup     & 91 & 94  & 95 & 97  & 90  & 98  & 99  & 100 & 100 \\
        Hang Mug             & 19 & 27  & 21 & 25  & 24  & 28  & 28  & 36  & 31  \\
        Unhang Mug           & 79 & 77  & 82 & 72  & 96  & 76  & 96  & 85  & 94  \\
        Rotate QR Code       & 55 & 55  & 65 & 80  & 69  & 78  & 79  & 88  & 75  \\
        Rotate QR Code Back  & 99 & 98  & 100 & 100 & 100 & 100 & 99  & 99  & 98  \\
        Handover Block       & 86 & 92  & 86 & 92  & 89  & 94  & 97  & 96  & 97  \\
        Handover Block Back  & 99 & 100 & 98 & 100 & 97  & 97  & 98  & 99  & 99  \\
        Open Laptop          & 70 & 81  & 89 & 93  & 85  & 81  & 97  & 97  & 86  \\
        Close Laptop         & 73 & 61  & 79 & 69  & 88  & 73  & 93  & 92  & 88  \\
        Open Microwave       & 72 & 83  & 86 & 96  & 80  & 73  & 95  & 98  & 92  \\
        Close Microwave      & 73 & 77  & 74 & 82  & 73  & 69  & 75  & 74  & 83  \\
        \midrule
        Macro average        & 67.5 & 73.3 & 74.6 & 78.4 & 77.3 & 77.2 & 83.2 & 85.2 & 85.4 \\
        \bottomrule
    \end{tabular}
\end{table*}

